Think Twice: Branch-and-Rethink Reasoning Reward Model

Large language models (LLMs) increasingly rely on thinking models that externalize intermediate steps and allocate extra test-time compute, with think-twice strategies showing that a deliberate second pass can elicit stronger reasoning. In contrast, most reward models (RMs) still compress many quality dimensions into a single scalar in one shot, a design that induces judgment diffusion: attention spreads across evaluation criteria, yielding diluted focus and shallow analysis. We introduce branch-and-rethink (BR-RM), a two-turn RM that transfers the think-twice principle to reward modeling. Turn 1 performs adaptive branching, selecting a small set of instance-critical dimensions (such as factuality and safety) and sketching concise, evidence-seeking hypotheses. Turn 2 executes branch-conditioned rethinking, a targeted reread that tests those hypotheses and scrutinizes only what matters most. We train with GRPO-style reinforcement learning over structured two-turn traces using a simple binary outcome reward with strict format checks, making the approach compatible with standard RLHF pipelines. By converting all-at-once scoring into focused, second-look reasoning, BR-RM reduces judgment diffusion and improves sensitivity to subtle yet consequential errors while remaining practical and scalable. Experimental results demonstrate that our model achieves state-of-the-art performance on three challenging reward modeling benchmarks across diverse domains.

==> table/comp_ab.tex <==
\renewcommand\arraystretch{1.1}
\begin{table}[ht!]
    \centering \small
    \tabcolsep0.075 in
    \caption{
        \textbf{Ablation Study.} This table summarizes the performance impact of removing key components from our BR-RM models. Values in parentheses show the performance drop from the full models, highlighting the contribution of each component. Due to space constraints, RewardBench is abbreviated as RB. The full results of different model sizes are in Table \ref{tab:comp_ablation_full}.
    }
    %\vspace{2mm}
    \label{tab:comp_ablation}
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2.5}{*}{\textbf{Prompting strategy}} & \multicolumn{4}{c}{\textbf{BR-RM-Qwen-14B}} \\
    \cmidrule(lr){2-5}
    & \textbf{RB} & \textbf{RMBench} & \textbf{RMB} & \textbf{Avg} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-5}
    \textbf{BR-RM (Full Model)}
    & \textbf{92.1} & \textbf{85.9} & \textbf{74.7} & \textbf{84.2} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-5}
    Branching Only
    & 90.9 & 83.2 & 71.0 & 81.7 \\
    Unconditioned Rethink
    & 91.3 & 84.4 & 71.9 & 82.5 \\
    Single-Turn Model
    & 91.3 & 85.2 & 73.3 & 83.3 \\
\bottomrule
%\vspace{-8mm}
\end{tabular}
\end{table}

==> table/data_ab.tex <==
\renewcommand\arraystretch{1.1}
\begin{table}[t]
    \centering \small
    \tabcolsep0.07 in
    %\vspace{-5mm}
    \caption{
        \textbf{Training Data Analysis.} Impact of training data sources for our BR-RM model (14B). Due to space constraints, RewardBench is abbreviated as RB. The full results of different model sizes are in Table \ref{tab:data_ablation_full}.
    }
    %\vspace{2mm}
    \label{tab:data_ablation}
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2.5}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{BR-RM-Qwen-14B}} \\
    \cmidrule(lr){2-5}
    & \textbf{RB} & \textbf{RMBench} & \textbf{RMB} & \textbf{Avg} \\
    % \midrule
    \cmidrule(lr){1-1} \cmidrule(lr){2-5}
    \textbf{Full training data}
    & \textbf{92.1} & \textbf{85.9} & \textbf{74.7} & \textbf{84.2} \\
    \quad w/o HelpSteer3
    & 91.5 & 84.4 & 70.3 & 82.1 \\
    \quad w/o Skywork
    & 91.3 & 85.1 & 69.7 & 82.0 \\
    \quad w/o Math-Step-DPO
    & 91.5 & 85.0 & 72.6 & 83.0 \\
    \quad w/o Code-Preference
    & 91.8 & 85.4 & 74.0 & 83.7 \\
    \bottomrule
    %\vspace{-5mm}
\end{tabular}
\end{table}

==> table/reward_ana.tex <==
\renewcommand\arraystretch{1.1}
\begin{table}[ht!]
    \centering \small
    \tabcolsep0.075 in
    \caption{
        \textbf{Reward Analysis.} Quantitative comparison of our proposed reward design against several ablations. Our approach using a direct binary reward consistently achieves the highest scores. Due to space constraints, RewardBench is abbreviated as RB.
    }
    %\vspace{2mm}
    \label{tab:reward_ana}
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2.5}{*}{\textbf{Reward}} & \multicolumn{4}{c}{\textbf{BR-RM-Qwen-14B}} \\
    \cmidrule(lr){2-5}
    & \textbf{RB} & \textbf{RMBench} & \textbf{RMB} & \textbf{Avg} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-5}
    \textbf{Our Reward}
    & \textbf{92.1} & \textbf{85.9} & \textbf{74.7} & \textbf{84.2} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-5}
    Removing Format Checks
    & 91.3 & 85.4 & 73.1 & 83.3 \\
    Scoring on a Scale
    & 90.8 & 85.1 & 71.7 & 82.5 \\
    Reward for Branch
    & 87.8 & 82.7 & 69.3 & 79.9 \\
    \bottomrule
    %\vspace{-5mm}
\end{tabular}
\end{table}
